Fractional Repetition Codes for Repair in Distributed Storage Systems

We introduce a new class of exact Minimum-Bandwidth Regenerating (MBR) codes for distributed storage systems, characterized by a low-complexity uncoded repair process that can tolerate multiple node failures. These codes consist of the concatenation of two components: an outer MDS code followed by an inner repetition code. We refer to the inner code as a Fractional Repetition code since it consists of splitting the data of each node into several packets and storing multiple replicas of each on different nodes in the system. Our model for repair is table-based, and thus, differs from the random access model adopted in the literature. We present constructions of Fractional Repetition codes based on regular graphs and Steiner systems for a large set of system parameters. The resulting codes are guaranteed to achieve the storage capacity for random access repair. The considered model motivates a new definition of capacity for distributed storage systems, that we call Fractional Repetition capacity. We provide upper bounds on this capacity while a precise expression remains an open problem.

==> RelatedWork.tex <==
 
\section{related Work}\label{sec:RelatedWork}
The pioneering work of Dimakis et al. in \cite{ DGWR07, DGWWR07,  WDR07}
 introduced  Regenerating codes for  distributed storage systems. The authors showed that there exists a tradeoff between  storage capacity and repair bandwidth in these systems. Moreover, they determined their storage capacity  using network coding techniques and showed that random linear network codes are optimal  under a functional repair model. 
  
  Subsequent works focused on the design of  Exact Regenerating codes    that can repair the system by regenerating an exact copy of the lost data. Rashmi et al. constructed Exact MBR codes  for the special case of $d=n-1$ \cite{RSKR09}, and   for all feasible values of the repair degree $d$ in \cite{RSKKisit}.
  The existence of Exact Regenerating  codes for another important regime, known as the Minimum Storage Regime (MSR),  was demonstrated in \cite{SR10, CJM10},  and  deterministic constructions  were investigated  in  \cite{RSKR09, WD09, SR09, SRKR10}. 
  % The design of Regenerating codes that can protect the distributed storage system from  eavesdropping  or data corruption by malicious adversaries  was studied in \cite{PRR10, PRR10journal, DDH10}.
